Direction-Adaptive Haar Framelets on Graphs

Haar framelets on graphs extract local differences at different scales by comparing signals from children of the same parent, but building a tree from edge connectivity alone can assign adjacent nodes with markedly different features to different parents, making these differences hard to capture in the finest-scale high-pass responses. Inspired by how classical directional wavelets analyze local variation in rotated coordinates, we propose direction-adaptive Haar framelets on graphs (DAHF), a framework that changes what Haar compares at each scale by adapting the partition tree. DAHF learns candidate directions from feature differences between adjacent nodes and builds the partition tree level by level, favoring structurally admissible groupings in which feature variation within the parent is concentrated along one direction. Following PEGFAN's Haar construction, the complete transform preserves the input signal's energy and supports exact reconstruction, and its node responses are permutation equivariant when the nodes and partition tree are relabeled together. For two stripe signals on a periodic grid, the fraction of energy entering the finest-scale high-pass band rises from about 43%-47% with PEGFAN using the Paris clustering method built into the authors' example code (Paris-PEGFAN) to 85%-86% with DAHF. Across nine node classification datasets, DAHF achieves an average accuracy of 69.09%, ranking first among the methods compared and exceeding preset Paris-PEGFAN by 0.75 percentage points.

==> figures/source/haar-regrouping.tex <==
\begin{figure}[t]
\centering
\definecolor{HaarTreeRed}{HTML}{B22222}
\definecolor{HaarTreeBlue}{HTML}{376B9E}
\begin{tikzpicture}[
    x=.74cm,
    y=.86cm,
    font=\footnotesize,
    cluster/.style={draw=HaarTreeBlue!65, rounded corners=2pt, fill=white, inner sep=3pt, line width=.5pt},
    leaf/.style={cluster, minimum width=7mm, minimum height=5mm},
    tree edge/.style={draw=HaarTreeBlue!70, line width=.6pt}]
    \node at (3,3.62) {Same node features \(y_1=y_2=a,\quad y_3=y_4=b,\quad a\ne b\)};
    \foreach \x/\heading/\firstpartner/\secondpartner/\result in {
        0/{(a) Edge-only pairing}/2/3/{=0},
        6/{(b) Directional grouping}/3/2/{\ne 0}} {
        \begin{scope}[shift={(\x,0)}]
            \path[fill=HaarTreeBlue!9,rounded corners=4pt]
                (-2.40,-2.50) rectangle (2.50,2.93);
            \path[fill=HaarTreeBlue!3,rounded corners=4pt]
                (-2.45,-2.45) rectangle (2.45,2.98);
            \path[fill=HaarTreeBlue!11,rounded corners=4pt]
                (-2.45,2.37) rectangle (2.45,2.98);
            \draw[HaarTreeBlue!22,line width=.4pt] (-2.45,2.37) -- (2.45,2.37);
            \draw[draw=HaarTreeBlue!50,rounded corners=4pt,line width=.5pt]
                (-2.45,-2.45) rectangle (2.45,2.98);
            \path[fill=white,rounded corners=3pt]
                (-2.23,-2.23) rectangle (2.23,-.55);
            \draw[HaarTreeRed!25,line width=.45pt] (-1.95,-.62) -- (1.95,-.62);
            \node[text=HaarTreeBlue!75!black] at (0,2.68) {\heading};
            \node[cluster,fill=HaarTreeBlue!7] (root) at (0,1.80) {\(\{1,2,3,4\}\)};
            \node[cluster]
                (left) at (-1.03,.85) {\(\{\textcolor{HaarTreeRed}{1},\textcolor{HaarTreeRed}{\firstpartner}\}\)};
            \node[cluster] (right) at (1.03,.85) {\(\{\secondpartner,4\}\)};
            \node[leaf] (a) at (-1.55,-.10) {\(\{1\}\)};
            \node[leaf] (b) at (-.52,-.10) {\(\{\firstpartner\}\)};
            \node[leaf] (c) at (.52,-.10) {\(\{\secondpartner\}\)};
            \node[leaf] (d) at (1.55,-.10) {\(\{4\}\)};
            \draw[tree edge] (root) -- (left) (root) -- (right)
                (left) -- (a) (left) -- (b) (right) -- (c) (right) -- (d);
            \node[text=HaarTreeRed,align=center] at (0,-1.48) {Finest-scale high-pass\\
                \(\displaystyle\frac{y_1-y_{\firstpartner}}{\sqrt{2}}\result\)};
        \end{scope}
    }
\end{tikzpicture}
\caption{Regrouping aligns the finest-scale Haar comparison with feature variation. Red digits mark the cluster containing node \(1\), and red text shows its high-pass response. In the left panel, pairing by edges alone groups nodes \(1\) and \(2\), whose features are equal, so the difference is zero. In the right panel, grouping by feature direction gives a high-pass response along \(a-b\) for nodes \(1\) and \(3\).}
\label{fig:haar-regrouping}
\end{figure}


==> figures/source/parent-construction.tex <==
\begin{figure*}[t]
\centering
\usetikzlibrary{shadows}
\colorlet{ParentDiagramBorder}{black!28}
\definecolor{ParentDiagramBlue}{HTML}{376B9E}
\definecolor{ParentDiagramRed}{HTML}{B22222}
\definecolor{ParentDiagramLightBlue}{HTML}{E4F1FF}
\definecolor{ParentDiagramPink}{HTML}{E5B5B5}
\setlength{\fboxsep}{7pt}
\setlength{\fboxrule}{0.5pt}
\newcommand{\parentPanelWidth}{\dimexpr\linewidth-2\fboxsep-2\fboxrule-34pt\relax}
% Enclose both parts of the figure in one rounded frame.
\newsavebox{\parentPanelBox}
\newcommand{\drawParentPanelFrame}{%
    \tikz{\node[draw=ParentDiagramBlue!55, fill=ParentDiagramBlue!3, rounded corners=5pt,
        drop shadow={shadow xshift=1pt,shadow yshift=-1.2pt,fill=ParentDiagramBlue!25,opacity=.22},
        line width=\fboxrule, inner sep=\fboxsep, outer sep=0pt]
        {\usebox{\parentPanelBox}};}%
}
\begin{lrbox}{\parentPanelBox}
\begin{minipage}{\parentPanelWidth}
\centering
\colorbox{ParentDiagramBlue!11}{\parbox{\dimexpr\linewidth-2\fboxsep\relax}{
    \centering\small\bfseries\color{ParentDiagramBlue!75!black} (a) Edge-based layerwise grouping}}\par
\vspace{8pt}
\begin{tikzpicture}[
    every node/.style={font=\small},
    member/.style={circle,draw=black!60,fill=white,minimum size=5.5mm,inner sep=0pt},
    panel/.style={draw=ParentDiagramBlue!35,fill=white,rounded corners=3pt,line width=.45pt,
        drop shadow={shadow xshift=.5pt,shadow yshift=-.6pt,fill=ParentDiagramBlue!20,opacity=.18}},
    stage/.style={font=\small\bfseries,text=ParentDiagramBlue!75!black},
    link/.style={draw=ParentDiagramBlue,semithick},
    flow/.style={->,thick,draw=black!65}]
    \draw[panel] (0,-.52) rectangle (4.10,3.24);
    \draw[panel] (4.62,-.52) rectangle (8.85,3.24);
    \draw[panel] (9.37,-.52) rectangle (14.60,3.24);
    % Use a soft band for the three structural steps.
    \path[fill=ParentDiagramBlue!9,rounded corners=3pt] (0,2.56) rectangle (4.10,3.24);
    \path[fill=ParentDiagramBlue!9,rounded corners=3pt] (4.62,2.56) rectangle (8.85,3.24);
    \path[fill=ParentDiagramBlue!9,rounded corners=3pt] (9.37,2.56) rectangle (14.60,3.24);
    \begin{scope}[xshift=2.05cm]
        \node[stage] at (0,2.88) {Find candidates};
        % Shrink the candidate illustration and align its opening text with the next card.
        \begin{scope}[shift={(0,-.011)},scale=.9,transform shape]
        \node at (0,2.39) {Selected children \(S=\{i,i'\}\)};
        \draw[draw=ParentDiagramBlue!55,fill=ParentDiagramLightBlue,rounded corners=3pt]
            (-1.56,1.37) rectangle (1.56,2.05);
        \node[member] (i) at (-1.08,1.71) {\(i\)};
        \node[member] (ip) at (1.08,1.71) {\(i'\)};
        \node[member] (j) at (-1.08,.36) {\(j\)};
        \node[member] (k) at (1.08,.36) {\(k\)};
        \draw[black!45] (i) -- (ip) (j) -- (k);
        \draw[link] (i) -- (j) (ip) -- (j) (ip) -- (k);
        \node at (0,-.18) {Unassigned neighbors \(j,k\)};
        \end{scope}
    \end{scope}
    \draw[flow] (4.16,1.3) -- (4.56,1.3);

    \begin{scope}[xshift=6.735cm]
        \node[stage] at (0,2.88) {Compute structural scores};
        \begin{scope}[yshift=-2.5mm]
            \node at (0,2.39) {For each candidate \(u\in\{j,k\}\)};
            \node at (0,1.03) {\(\begin{aligned}
                w(S,u)&=A_{iu}^{(\ell)}+A_{i'u}^{(\ell)},\\[3pt]
                P_\ell(S,u)&=\frac{T_\ell w(S,u)}{v_S v_u}.
            \end{aligned}\)};
        \end{scope}
    \end{scope}
    \draw[flow] (8.91,1.3) -- (9.31,1.3);

    \begin{scope}[xshift=11.985cm]
        \node[stage] at (0,2.88) {Apply the structural threshold};
        \begin{scope}[yshift=-2.5mm]
            \node at (0,2.30) {\(P_{\max}=\max\{P_\ell(S,j),P_\ell(S,k)\}\)};
            \node[draw=ParentDiagramBlue!55,fill=ParentDiagramLightBlue,rounded corners=2pt,inner sep=4pt]
                at (0,1.42) {\(P_\ell(S,u)\geq\tau P_{\max}\)};
            \node at (0,.56) {Score retained candidates by direction};
        \end{scope}
    \end{scope}
\end{tikzpicture}
\par\nointerlineskip\vspace{10pt}
\begin{tikzpicture}
    \draw[ParentDiagramBlue!45,dash pattern=on 3pt off 3pt,line width=.45pt]
        (0,0) -- (\dimexpr\linewidth-12pt\relax,0);
\end{tikzpicture}
\par\nointerlineskip\vspace{10pt}
\colorbox{ParentDiagramBlue!11}{\parbox{\dimexpr\linewidth-2\fboxsep\relax}{
    \centering\small\bfseries\color{ParentDiagramBlue!75!black} (b) Direction-adaptive grouping}}\par
\vspace{8pt}
% Reuse the coordinate frame for the direction dictionary and both comparisons.
\newcommand{\drawParentCoordinateFrame}{%
    \coordinate (candidate origin) at (-1.925,.66);
    \draw[axis] (-2.72,.66) -- (-.30,.66);
    \draw[axis] (-1.925,.18) -- (-1.925,1.78);
}
\newcommand{\drawParentCandidateAxes}[1]{%
    \drawParentCoordinateFrame
    \draw[best axis] (candidate origin) -- ++(#1:1.12cm);
    \path (candidate origin) ++(210:.275cm) node[existing,label=below:\(i\)] {};
    \path (candidate origin) ++(30:.275cm) node[existing,label=below:\(i'\)] {};
}
\begin{tikzpicture}[
    every node/.style={font=\small},
    panel/.style={draw=ParentDiagramBlue!35,fill=white,rounded corners=3pt,line width=.45pt,
        drop shadow={shadow xshift=.5pt,shadow yshift=-.6pt,fill=ParentDiagramBlue!20,opacity=.18}},
    axis/.style={->,draw=black!40,thin},
    best axis/.style={->,draw=ParentDiagramBlue,very thick},
    existing/.style={circle,fill=ParentDiagramBlue,inner sep=0pt,minimum size=4pt},
    candidate/.style={circle,fill=ParentDiagramRed,inner sep=0pt,minimum size=5pt},
    flow/.style={->,semithick,draw=black!60}]
    \node[anchor=north west,inner sep=0pt,text width=9.30cm,align=left]
        at (-7.28,4.49) {Selected children \(S=\{i,i'\}\). Candidates \(j,k\) pass the structural threshold.};
    \node[anchor=north west,inner sep=0pt,text width=9.30cm,align=left]
        at (-7.28,3.47) {For each proposed parent \(U\), compute the share of variation along each axis, \(E_r(U)/E(U)\).};

    \begin{scope}[shift={(7.30,2.65)}]
        \draw[draw=ParentDiagramBlue!55,fill=ParentDiagramBlue!6,dashed,rounded corners=3pt] (-3.80,0) rectangle (0,2.00);
        \node at (-1.90,1.70) {Candidate directions};
        \begin{scope}[shift={(-.62,.01)},scale=.81]
            \drawParentCoordinateFrame
            \draw[best axis] (candidate origin) -- ++(30:1.12cm)
                node[right,text=ParentDiagramBlue] {\(q_1\)};
            \draw[best axis] (candidate origin) -- ++(60:1.12cm)
                node[right,inner sep=2pt,text=ParentDiagramBlue] {\(q_2\)};
        \end{scope}
    \end{scope}

    \begin{scope}[xshift=-3.75cm]
        \draw[panel] (-3.55,-.30) rectangle (3.55,2.39);
        \node[text=ParentDiagramBlue!75!black] at (0,1.99) {Try \(j\) to form \(U_j=S\cup\{j\}\)};
        \drawParentCandidateAxes{30}
        \path (candidate origin) ++(30:.95cm) node[candidate,label=below:\(j\)] {};
        \node[text=ParentDiagramBlue] at (-.94,1.42) {\(q_1\)};
        \node at (1.18,1.26) {Best axis: \(q_1\)};
        \node at (1.18,.61) {\(\displaystyle C(U_j)=\frac{E_1(U_j)}{E(U_j)}\)};
    \end{scope}

    \begin{scope}[xshift=3.75cm]
        \draw[panel] (-3.55,-.30) rectangle (3.55,2.39);
        \node[text=ParentDiagramBlue!75!black] at (0,1.99) {Try \(k\) to form \(U_k=S\cup\{k\}\)};
        \drawParentCandidateAxes{60}
        \path (candidate origin) ++(60:.84cm) node[candidate,label=right:\(k\)] {};
        \node[text=ParentDiagramBlue] at (-1.79,1.62) {\(q_2\)};
        \node at (1.18,1.26) {Best axis: \(q_2\)};
        \node at (1.18,.61) {\(\displaystyle C(U_k)=\frac{E_2(U_k)}{E(U_k)}\)};
    \end{scope}

    \node[draw=ParentDiagramPink!78!black,fill=ParentDiagramPink!28,rounded corners=3pt,inner sep=5pt]
        at (0,-1.08) {Compare scores: \(C(U_j)>C(U_k)\), so add \(j\) to \(S\).};
    \draw[flow] (-3.75,-.35) -- (-1.95,-.76);
    \draw[flow] (3.75,-.35) -- (1.95,-.76);
\end{tikzpicture}
\end{minipage}
\end{lrbox}
\drawParentPanelFrame
\caption{One step of growing a parent at level \(\ell+1\). (a) The selected children inside the box and the candidates connected by blue edges are all at level \(\ell\). (b) The upper-right inset shows two candidate directions from the dictionary. The two panels below use the same feature coordinates. Blue dots indicate the selected children, red dots indicate the candidates being considered, and blue arrows mark the highest-scoring direction for each grouping. After comparing the two directional scores, we add \(j\) to \(S\).}
\label{fig:parent-construction}
\end{figure*}

